Sequential Decision Making with Expert Demonstrations under Unobserved Heterogeneity

We study the problem of online sequential decision-making given auxiliary demonstrations from experts who made their decisions based on unobserved contextual information. These demonstrations can be viewed as solving related but slightly different problems than what the learner faces. This setting arises in many application domains, such as self-driving cars, healthcare, and finance, where expert demonstrations are made using contextual information, which is not recorded in the data available to the learning agent. We model the problem as zero-shot meta-reinforcement learning with an unknown distribution over the unobserved contextual variables and a Bayesian regret minimization objective, where the unobserved variables are encoded as parameters with an unknown prior. We propose the Experts-as-Priors algorithm (ExPerior), an empirical Bayes approach that utilizes expert data to establish an informative prior distribution over the learner's decision-making problem. This prior distribution enables the application of any Bayesian approach for online decision-making, such as posterior sampling. We demonstrate that our strategy surpasses existing behaviour cloning, online, and online-offline baselines for multi-armed bandits, Markov decision processes (MDPs), and partially observable MDPs, showcasing the broad reach and utility of ExPerior in using expert demonstrations across different decision-making setups.

==> sections/appx_regret.tex <==
\section{Regret Analysis for Max-Entropy Posterior Sampling}
\subsection{Setting} Here, we focus a the general setting called Decision Making with Structured Observations (DMSO) \citep{foster2021statistical}. For a particular decision-making task, consider $T$ episodes, where at each episode $t = 1, \ldots, T:$
\begin{enumerate}
    \item The agent selects a decision $\decision^t \in \decSpace$, where $\decSpace$ is a decision space.
    \item Nature selects a reward $r^t \in \cR$ and observation $o^t \in \cO$ based on the decision, where $\cR \subseteq \R$ is the reward space and $\cO$ is the observation space. The reward and observation are observed by the agent.
\end{enumerate}
We make the following assumptions for the DMSO framework.
\begin{assumption}[Stochastic DMSO with Finite Decisions] \label{assump:stochastic-dmso} We assume that the reward space is bounded $\cR = [0, 1]$, the decision space $\decSpace$ is finite, and for a particular task, the rewards and observations are generated independently via
\begin{align}
    (r^t, o^t) \sim M_\theta\lpar \cdot \given \decision^t \rpar,
\end{align}
where $M_\theta: \decSpace \to \Delta(\cR \times \cO)$ is the underlying model parameterized by $\theta \in \Theta$. Moreover, $\theta$ is a random variable indicating the task. In particular, we assume an unknown (prior) distribution $\mu^\star \in \Delta(\Theta)$ over the decision-making tasks $\Theta$. Finally, the model class $\lcbar M_\theta \midsem \theta \in \Theta \rcbar$ is known to the agent.
\end{assumption}

Denote the mean reward function under $(r, o) \sim M_\theta(\decision)$ by
\begin{align}
    f^\theta(\decision) := \E_{r \sim M_\theta(\decision)} \lpar r \rpar,
\end{align}
and the optimal decision for model $M_\theta$ by\footnote{For simplicitly of our analysis, we assume the optimal decision is unique.}
\begin{align}
    \decision_\theta := \argmax_{\decision \in \decSpace} f^\theta(\decision).
\end{align}
The agent's goal is to learn a history-dependent distribution over decisions $p^1, \ldots, p^T \in \Delta(\decSpace)$ to minimize the Bayesian regret:
\begin{align}
    \bregret := \E_{\theta \sim \mu^\star} \lbar \sum_{t=1}^T  f^\theta(\decision_\theta) - \E_{\decision^t \sim p^t} \lbar f^\theta(\decision^t)\rbar \rbar. \label{eq:bayes-regret} 
\end{align}

\subsection{Information-theoretic regret analysis for posterior sampling with misspecified prior}
Consider a history of agent's interaction with the environment up to episode $t$ as $h_{t-1} = \{\decision^1, r^1, o^1, \ldots, \decision^{t-1}, r^{t-1}, o^{t-1}\}$. Given $h_{t-1}$, a posterior-sampling agent takes a decision with the posterior probability of optimal policy under a (potentially misspecified) prior $\mu$, i.e.,  $p^t(\decision) = \mu \lpar \decision_\theta = \decision \given h_{t-1}\rpar$. For this strategy, we prove the following lemma that bounds the Bayesian regret based on the distance between the posterior distribution under the true prior $\mu^\star\lpar \cdot \given h_{t-1}\rpar$ and the agent's prior $\mu\lpar \cdot \given h_{t-1}\rpar$. To simplify the notation, we denote the posterior distributions at time $t$ by $\mu^\star_t$ and $\mu_t$, and the expectation evaluated under the posterior measure $\mu^\star_t$ as $\E_t$.
\begin{lemma} \label{lemma:bound-mis-prior}
    Under \cref{assump:stochastic-dmso}, the Bayesian regret \cref{eq:bayes-regret} of a posterior-sampling agent with prior a $\mu$ such that $\mu^\star \ll \mu$ is bounded by
    \begin{align}
        \bregret \leq \E \lbar  \sum_{t=1}^T \tv{\mu_t}{\mu_t^\star}\rbar + \sqrt{\frac12 \E \lbar \sum_{t=1}^T {\Gamma_t}\rbar \cdot \entropy^*(\decision_\theta)}, \label{eq:bound-mis-prior}
    \end{align}
    where $\Gamma_t := \sum_{\decision \in \decSpace} \frac{\mu^\star_t\left(\decision_\theta = \decision\right)}{\mu_t\left(\decision_\theta = \decision\right)}$, $\entropy^*(\decision_\theta)$ is the entropy of the optimal decision under the true prior distribution $\mu^\star$, and the expectations are taken over the history of agent's interaction with the environment.
\end{lemma}
\begin{proof}
We start by simplifying \cref{eq:bayes-regret}:
{\small
\begin{align}
     \bregret &= \E \lbar \sum_{t=1}^T \E_t \lbar f^\theta(\decision_\theta)-  \E_{\decision^t \sim p^t} \lbar f^\theta(\decision^t)\rbar \rbar \rbar \tag{By law of total expectation}\\
     &= \E \lbar \sum_{t=1}^T \E_t \lbar f^\theta(\decision_\theta)-  \sum_{\decision \in \decSpace} p^t(\decision) f^\theta(\decision) \rbar \rbar\\
     &= \E  \lbar \sum_{t=1}^T \sum_{\decision \in \decSpace} \mu^\star_t\lpar \decision_\theta = \decision \rpar \E_t\lbar f^\theta(\decision) \given \decision_\theta = \decision\rbar - p^t(\decision) \E_t \lbar f^\theta(\decision) \rbar \rbar.
\end{align}
}%
Adding and subtracting $\mu_t^\star\lpar \decision_\theta = \decision \rpar \E_t\lbar f^\theta(\decision)\rbar$ to the sum above, we get
{\small
\begin{align}
     \bregret
     &= \underbrace{\E  \lbar \sum_{t=1}^T\sum_{\decision \in \decSpace} \mu_t^\star\lpar \decision_\theta = \decision \rpar \lpar \E_t\lbar f^\theta(\decision) \given \decision_\theta = \decision\rbar - \E_t \lbar f^\theta(\decision) \rbar \rpar  \rbar}_{(1)} + \underbrace{\E  \lbar \sum_{t=1}^T \sum_{\decision\in \decSpace}  \lpar \mu_t^\star\lpar \decision_\theta = \decision\rpar - p^t(\decision) \rpar  \E_t\lbar f^\theta(\decision)\rbar \rbar}_{(2)}.
\end{align}
}%
\xhdr{Bounding (1)} $\mu^\star \ll \mu$ implies that $\mu^\star_t \ll \mu_t$. Therefore, $\frac{\mu^\star_t\left(\decision_\theta = \decision\right)}{\mu_t\left(\decision_\theta = \decision\right)}$ is well-defined for all $\decision \in \decSpace$. Recalling that $p^t(\decision) = \mu_t(\decision_\theta = \decision)$, we get
{\small
\begin{align}
     (1) &=  \E  \lbar \sum_{t=1}^T \sum_{\decision \in \decSpace} \sqrt{\frac{\mu^\star_t\lpar \decision_\theta = \decision \rpar}{p^t(\decision)}} \sqrt{\mu^\star_t\lpar \decision_\theta = \decision \rpar p^t(\decision)} \lpar \E_t\lbar f^\theta(\decision) \given \decision_\theta = \decision \rbar - \E_t \lbar f^\theta(\decision) \rbar \rpar \rbar \\
      & \stackrel{(a)}{\leq}  \E  \lbar \sum_{t=1}^T \sqrt{\sum_{\decision \in \decSpace} {\frac{\mu^\star_t\lpar \decision_\theta = \decision \rpar}{p^t(\decision)}}} \cdot \sqrt{\sum_{\decision \in \decSpace} {\mu^\star_t\lpar \decision_\theta = \decision \rpar p^t(\decision)} \lpar \E_t\lbar f^\theta(\decision) \given \decision_\theta = \decision\rbar - \E_t \lbar f^\theta(\decision) \rbar \rpar^2} \rbar, \label{eq:help-bregret}
\end{align}
}%
where (a) follows form the Cauchy-Schwarz inequality. Now, note that
{\small
\begin{align}
    \E_t\lbar f^\theta(\decision) \given \decision_\theta = \decision \rbar - \E_t \lbar f^\theta(\decision) \rbar  &= \E_t\lbar r^t \given \decision_\theta = \decision, \decision^t = \decision \rbar - \E_t \lbar r^t \given \decision^t = \decision\rbar \\
    & \stackrel{(a)}{\leq} \sqrt{\frac12 \kl{\mu^\star_t\lpar r^t \given \decision_\theta = \decision, \decision^t = \decision\rpar}{\mu_t^\star\lpar r^t \given \decision^t = \decision\rpar}} ,\label{eq:pinsker-bregret}
\end{align}
}%
where (a) follows from Pinsker's inequality since $\cR = [0, 1]$.

Combining \cref{eq:help-bregret,eq:pinsker-bregret} and noting that $\Gamma_t = \sum_{\decision \in \decSpace} {\frac{\mu_t^\star\lpar \decision_\theta = \decision \rpar}{p^t(\decision)}}$, we get
{\small
\begin{align}
    (1) & \leq \E  \lbar \sum_{t=1}^T \sqrt{\Gamma_t} \cdot \sqrt{\frac12 \sum_{\decision \in \decSpace}  {\mu^\star_t\lpar \decision_\theta = \decision \rpar p^t(\decision)} \kl{\mu^\star_t\lpar r^t \given \decision_\theta = \decision, \decision^t = \decision\rpar}{\mu_t^\star\lpar r^t \given \decision^t = \decision\rpar} } \rbar \\
    & \stackrel{(a)}{\leq} \E  \lbar \sum_{t=1}^T \sqrt{\Gamma_t} \cdot \sqrt{\frac12 I_t^\star\lpar \decision_\theta ; \decision^t, r^t \rpar} \rbar \\
    & {\leq} \sqrt{\frac12 \E  \lbar \sum_{t=1}^T {\Gamma_t}\rbar \cdot \E \lbar{\sum_{t=1}^T I_t^\star \lpar \decision_\theta ; \decision^t, r^t \rpar} \rbar} \tag{By Cauchy-Schwarz}\\
    & \stackrel{(b)}{\leq} \sqrt{\frac12 \E  \lbar \sum_{t=1}^T {\Gamma_t}\rbar \cdot \entropy^\star(\decision_\theta)}  \label{eq:term-i}
\end{align}
}%
where $I_t^\star\lpar \decision_\theta ; \decision^t, r^t\rpar$ is the mutual information between the optimal action $\decision_\theta$ and the observed action/reward at time $t$ under the posterior distribution $\mu_t^\star$, and $\entropy^\star(\decision_\theta)$ is the entropy of the optimal decision under the prior distribution. To see why (a) holds, note that
{\small
\begin{align}
    I^\star_t\lpar \decision_\theta \midsem \decision^t, r^t \rpar &= I^\star_t\lpar \decision_\theta \midsem \decision^t \rpar + I^\star_t\lpar \decision_\theta \midsem  r^t \given \decision^t\rpar \tag{By chain rule for mutual information} \\
    & = I^\star_t\lpar \decision_\theta \midsem  r^t \given \decision^t\rpar \tag{Since $\decision^t$ and $\decision_\theta$ are independent given history}\\
    & = \sum_{\decision \in \decSpace} p^t(\decision) I^\star_t\lpar \decision_\theta \midsem  r^t \given \decision^t = \decision \rpar \\
    & = \sum_{\decision \in \decSpace} p^t(\decision) \E_{\decision_\theta} \lbar \kl{\mu_t^\star\lpar r^t \given \decision_\theta, \decision^t = \decision \rpar}{\mu_t^\star\lpar r^t \given  \decision^t = \decision \rpar} \rbar \\
    & = \sum_{\decision \in \decSpace} \sum_{\decision' \in \decSpace} p^t(\decision) \mu^\star_t\lpar \decision_\theta = \decision' \rpar \kl{\mu_t^\star\lpar r^t \given \decision_\theta = \decision', \decision^t = \decision \rpar}{\mu_t^\star\lpar r^t \given  \decision^t = \decision \rpar} \\
    & \geq \sum_{\decision \in \decSpace}  p^t(\decision) \mu^\star_t\lpar \decision_\theta = \decision \rpar \kl{\mu_t^\star\lpar r^t \given \decision_\theta = \decision, \decision^t = \decision \rpar}{\mu_t^\star\lpar r^t \given  \decision^t = \decision \rpar}.
\end{align}
}%
To prove (b), we note that
{\small
\begin{align}
    \E \lbar{\sum_{t=1}^T I_t^\star \lpar \decision_\theta ; \decision^t, r^t \rpar} \rbar = \sum_{t=1}^T \E \lbar{I_t^\star \lpar \decision_\theta ; \decision^t, r^t \rpar} \rbar &= \sum_{t=1}^T I^\star \lpar \decision_\theta ; \lpar \decision^t, r^t\rpar \given \lpar \decision^1, r^1\rpar , \ldots, \lpar\decision^{t-1}, r^{t-1}\rpar \rpar \\
    & = I^\star \lpar \decision_\theta \midsem \lpar \decision^1, r^1\rpar , \ldots, \lpar\decision^{T}, r^{T}\rpar \rpar \tag{By chain rule} \\
    & \leq \entropy^\star\lpar \decision_\theta \rpar.
\end{align}
}%

\xhdr{Bounding (2)} Recall that $p^t(\decision) = \mu_t\lpar \decision_\theta = \decision \rpar$. Therefore,
{\small
\begin{align}
(2) &= \E  \lbar \sum_{t=1}^T \sum_{\decision\in \decSpace}  \lpar \mu_t^\star\lpar \decision_\theta = \decision\rpar - \mu_t\lpar \decision_\theta = \decision \rpar \rpar  \E_t\lbar f^\theta(\decision)\rbar \rbar\\
& = \E  \lbar \sum_{t=1}^T \E_{\theta \sim \mu^\star_t}\lbar \sum_{\decision \in \decSpace} \E_t \lbar f^\theta(\decision) \rbar \cdot \bbI\lpar \decision_\theta = \decision \rpar\rbar - \E_{\theta \sim \mu_t}\lbar \sum_{\decision \in \decSpace} \E_t \lbar f^\theta(\decision) \rbar \cdot \bbI\lpar \decision_\theta = \decision \rpar \rbar\rbar \\
& = \E  \lbar \sum_{t=1}^T \E_{\theta \sim \mu^\star_t}\lbar g_t(\theta) \rbar - \E_{\theta \sim \mu_t}\lbar g_t(\theta) \rbar\rbar \tag{Setting $g_t(\theta) = \sum_{\decision \in \decSpace} \E_t \lbar f^\theta(\decision) \rbar \cdot \bbI\lpar \decision_\theta = \decision \rpar$ } \\
& \stackrel{(a)}{\leq} \E \lbar  \sum_{t=1}^T \tv{\mu_t}{\mu_t^\star}\rbar,
\label{eq:term-ii} 
\end{align}
}%
where (a) holds since $g_t: \Theta \to \cR = [0, 1]$. Combining \cref{eq:term-i,eq:term-ii} concludes the proof.
\end{proof}

\subsection{Regret bound for posterior sampling with uniform prior}
The regret bound in \cref{lemma:bound-mis-prior} holds for any arbitrary prior $\mu$ as long as $\mu^\star \ll \mu$. However, it might be the case that $\Gamma_t$ is not bounded under a particular choice of $\mu$, or the total variation distance between the true posterior and the misspecified posterior might be vacuous. This sections provides a concrete regret bound for the specific choice of an uninformative prior on $\Theta$. In particular, we first make the following assumption on the independence of the decision arms in our model:
\begin{assumption}[Independence of Decisions] \label{assump:indep-arms}
    We assume the decisions are independent, i.e., $\Theta = \bigotimes_{\decision \in \decSpace} \Theta_{\decision}$, where each $\Theta_\decision \subset \R$ is a \textit{bounded} parameter space corresponding to decision $\decision$, and $M_\theta(\decision) = M_{\theta_\decision}(\decision)$ for all $\decision \in \decSpace$ and $\theta = \lpar \theta_\decision\rpar_{\decision \in \decSpace} \in \Theta$. Moreover, we assume the prior is a product measure $\mu^\star(\theta) = \prod_{\decision \in \decSpace} \mu^\star_\decision(\theta_{\decision})$.
\end{assumption}
Given \cref{assump:indep-arms}, we choose a uniform prior density function as our uninformative prior:
\begin{definition}[Uniform Prior]\label{def:unif-prior}
    Let $\mu_0$ be the Lebesgue measure on $\R$. For any $ \decision \in \decSpace$ and $\theta_\decision \in \Theta_\decision$, define $\mu^\unif_\decision(\theta_\decision) = \frac{1}{\mu_0(\Theta_\decision)}$. A uniform prior $\mu^\unif \in \Delta(\Theta)$ is then defined as $\mu^\unif(\theta) = \prod_{\decision\in \decSpace} \mu^\unif_\decision(\theta_\decision)$ for all $\theta = \lpar \theta_\decision\rpar_{\decision \in \decSpace} \in \Theta$.
\end{definition}
In addition to \cref{assump:indep-arms}, we consider the following regularity assumption on the true prior $\mu^\star$. Before stating the assumption, we define the following:
\begin{definition}[$L^1$-Sobelov Space of Order $\alpha$]
    For an open interval $\cX \subseteq \R$, and $\alpha \in \N$, we call
    \begin{align}
         W^{1,\alpha}(\cX) := \lcbar f \in L^1\lpar\cX, \mu_0\rpar:\ D^j f\in L^1\lpar\cX, \mu_0\rpar \forall j = 1, \ldots, \alpha, \ \left\|f\right\|_{W^{1,\alpha}(\cX)} := \left\| f \right\|_1 + \left\|D^\alpha f\right\|_1 < \infty \rcbar
    \end{align}
    the $L^1$-Sobelov space of order $\alpha$, where $D^j f$ is the $j$th weak derivative of $f$.
\end{definition}

\begin{assumption}[Smoothness of the Prior and Likelihood Model]\label{assump:smooth-prior}~
\begin{enumerate} \setlength \itemsep{0.3em}
    \item The true prior density function (w.r.t. the Lebesgue measure) is bounded, i.e., $\left\|\mu^\star\right\|_\infty \leq B$.
    \item For all $\decision \in \decSpace$, we assume $\mu^\star_\decision$ is differentiable with a bounded derivative $\left\|(\mu^\star_\decision)'\right\|_\infty \leq B'$.
    \item For all $\decision \in \decSpace$, $\mu^\star_\decision \in W^{1, \alpha}\lpar \Theta_\decision \rpar$ for some $\alpha \geq 2$.
    \item For all $\decision \in \decSpace$ and all $(r, o) \in \cR \times \cO$, we have $M_{\theta_\decision}\lpar r, o \given \decision \rpar: \Theta_\decision \to \R \in  W^{1, \alpha}\lpar \Theta_\decision \rpar$ for some $\alpha \geq 2$.
\end{enumerate}
\end{assumption}

\begin{proof}
    Before starting the proof, we set up some notation. For a given history $h_{t} = \lcbar \lpar \decision^j, r^j, o^j\rpar\rcbar_{j=1}^{t}$, we define $h^\decision_{t} := \lcbar (r^j, o^j) \in h_{t}\midsem \decision^j = \decision\rcbar$ and $n_t(\decision) = \left| h^\decision_t \right|$ for all $\decision \in \decSpace$. Moreover, given a model $\theta \in \Theta$, we denote the likelihood of $h_{t}$ under $\theta$ by
    \begin{align}
        \ell_\theta(h_{t}) = \prod_{\decision \in \decSpace}\ \prod_{(r, o) \in h^\decision_{t}}M_{\theta_\decision} \lpar r, o \given \decision \rpar.
    \end{align}
    Finally, for a given prior density function $\mu \in \Delta(\Theta)$, we define
    \begin{align}
        \mu\lpar h_{t} \rpar := \E_{\theta \sim \mu}\lbar \ell_{\theta}\lpar h_{t}\rpar\rbar.
    \end{align}
     Note that $\mu^\star \ll \mu^\unif$, therefore we can use \cref{lemma:bound-mis-prior} to get
    \begin{align}
        \bregret \leq \E \lbar  \sum_{t=1}^T \tv{\mu^\unif_t}{\mu_t^\star}\rbar + \sqrt{\frac12 \E \lbar \sum_{t=1}^T {\Gamma_t}\rbar \cdot \entropy^*(\decision_\theta)}.
    \end{align}
    \xhdr{Bounding $\E \lbar \sum_{t=1}^T {\Gamma_t}\rbar$}  Recall that 
\begin{align}
    \Gamma_t = \sum_{\decision \in \decSpace} \frac{\mu_t^\star\lpar \decision_\theta = \decision\rpar}{\mu_t^\unif\lpar \decision_\theta = \decision\rpar} &= \sum_{\decision \in \decSpace} \frac{\E_{\theta \sim \mu^\star}\lbar \bbI\lpar \decision_\theta = \decision\rpar \cdot \ell_\theta\lpar h_{t-1}\rpar \rbar / \mu^\star\lpar h_{t-1} \rpar}{\E_{\theta \sim \mu^\unif}\lbar \bbI\lpar \decision_\theta = \decision\rpar  \cdot \ell_\theta\lpar h_{t-1}\rpar \rbar / \mu^\unif\lpar h_{t-1} \rpar} \\
    &= \frac{\mu^\unif\lpar h_{t-1} \rpar}{ \mu^\star\lpar h_{t-1} \rpar}\sum_{\decision \in \decSpace} \frac{\E_{\theta \sim \mu^\star}\lbar \bbI\lpar \decision_\theta = \decision\rpar \cdot \ell_\theta\lpar h_{t-1}\rpar \rbar }{\E_{\theta \sim \mu^\unif}\lbar \bbI\lpar \decision_\theta = \decision\rpar  \cdot \ell_\theta\lpar h_{t-1}\rpar \rbar}\\
    & \leq \frac{\mu^\unif\lpar h_{t-1} \rpar}{ \mu^\star\lpar h_{t-1} \rpar}\sum_{\decision \in \decSpace} \frac{\left\|\frac{\mu^\star}{\mu^\unif}\right\|_\infty \cdot \E_{\theta \sim \mu^\unif}\lbar \bbI\lpar \decision_\theta = \decision\rpar \cdot \ell_\theta\lpar h_{t-1}\rpar \rbar }{\E_{\theta \sim \mu^\unif}\lbar \bbI\lpar \decision_\theta = \decision\rpar  \cdot \ell_\theta\lpar h_{t-1}\rpar \rbar} \tag{By Hölder's inequality} \\
    & =  \left|\decSpace\right| \frac{\mu^\unif\lpar h_{t-1} \rpar}{ \mu^\star\lpar h_{t-1} \rpar}  \left\|\frac{\mu^\star}{\mu^\unif}\right\|_\infty \stackrel{(a)}{\leq} B\left|\decSpace\right| \frac{\mu^\unif\lpar h_{t-1} \rpar}{ \mu^\star\lpar h_{t-1} \rpar}  \prod_{\decision\in \decSpace} \mu_0\lpar \Theta_\decision\rpar,
    \label{eq:help-bound-gamma}
\end{align}
where inequality (a) follows from \cref{def:unif-prior,assump:smooth-prior}.

Define the space of all histories up to episode $t$ as $\cH_{t-1}$. Taking the expectation of \cref{eq:help-bound-gamma} over the histories $h_{t-1}$, we get
\begin{align}
    \E\lbar \Gamma_t \rbar &= \int_{\cH_{t-1}} \Gamma_t \cdot \mu^\star\lpar h_{t-1}\rpar \diff h_{t-1} \\
    & \leq B\left|\decSpace\right|\prod_{\decision\in \decSpace} \mu_0\lpar \Theta_\decision\rpar \int_{\cH_{t-1}} \frac{\mu^\unif\lpar h_{t-1} \rpar}{ \mu^\star\lpar h_{t-1} \rpar} \mu^\star\lpar h_{t-1}\rpar \diff h_{t-1} \tag*{By \cref{eq:help-bound-gamma}} \\
    & \leq B\left|\decSpace\right|\prod_{\decision\in \decSpace} \mu_0\lpar \Theta_\decision\rpar \int_{\cH_{t-1}} \lpar \int_{\Theta} \ell_{\theta}\lpar h_{t-1} \rpar \diff \mu_0 \rpar \diff h_{t-1} \\
    & = B\left|\decSpace\right|\prod_{\decision\in \decSpace} \mu_0\lpar \Theta_\decision\rpar \int_{\Theta} \int_{\cH_{t-1}}   \ell_{\theta}\lpar h_{t-1} \rpar \diff h_{t-1} \diff \mu_0 \\
    & = B\left|\decSpace\right|\prod_{\decision\in \decSpace} \mu_0\lpar \Theta_\decision\rpar, \label{eq:bound-gamma}
\end{align}
where the last equality holds since $\int_{\cH_{t-1}}   \ell_{\theta}\lpar h_{t-1} \rpar \diff h_{t-1} = 1$.

\xhdr{Bounding $\E \lbar \sum_{t=1}^T \tv{\mu^\unif_t}{\mu_t^\star}\rbar$} First, note that since both priors $\mu^\star$ and $\mu^\unif$ are product measures, and the decisions under the likelihood model are independent, the posterior distributions $\mu_t^\star$ and $\mu_t^\unif$ are also product measures, i.e., for any $\theta \in \Theta$, we have
\begin{align}
    \mu^\unif_t(\theta) = \prod_{\decision \in \decSpace} \mu^\unif_{\decision,t}(\theta_\pi), \text{ and} \quad \mu^\star_t(\theta) = \prod_{\decision \in \decSpace} \mu^\star_{\decision,t}(\theta_\pi),
\end{align}
where $\mu^\unif_{\decision,t}$ and $\mu^\star_{\decision,t}$ are the posterior density functions under the priors $\mu^\unif_\decision$ and $\mu^\star_\decision$. We now use the fact that the total variation distance between two product measures is bounded by the sum of their marginal distances as follows:
\begin{align}
    \tv{\mu^\unif_t}{\mu_t^\star} \leq \sum_{\decision \in \decSpace} \tv{\mu^\unif_{\decision,t}}{\mu_{\decision,t}^\star}. \label{eq:tv-product}
\end{align}
Before continuing the proof, we state and prove the following lemma that bounds the total variation distance between posterior distributions by the Wasserstein distance. 
\begin{lemma}[Wasserstein Bound for Total Variation]\label{lemma:wass-tv}
    Under \cref{assump:smooth-prior}, for all $\decision \in \decSpace$, we have
    \begin{align}
        \tv{\mu^\unif_{\decision,t}}{\mu_{\decision,t}^\star} \leq c \lpar \left\|\mu^\unif_{\decision,t}\right\|_{W^{1,\alpha}} + \left\|\mu^\star_{\decision,t}\right\|_{W^{1,\alpha}}\rpar^{\frac{1}{\alpha+1}} \lpar\wass{\mu^\unif_{\decision,t}}{\mu_{\decision,t}^\star}\rpar^{\frac{\alpha}{\alpha + 1}}, \label{eq:wass-tv}
    \end{align}
    where $c > 0$ is a constant depending only on $\alpha$ and $\mathrm{D}_\mathrm{W}$ is the 1-Wasserstein distance.
\end{lemma}
\begin{proof}
    First, we prove that the posterior density functions $\mu^\unif_{\decision,t}$ and $\mu_{\decision,t}^\star$ belong to $W^{1,\alpha}\lpar \Theta_\decision \rpar$. To see this, note that
    \begin{align}
        \mu_{\decision,t}^\star(\theta_\decision) = \kappa \mu_\decision^\star(\theta_\decision) \prod_{(r, o) \in h^\decision_{t-1}} M_{\theta_\decision}\lpar r, o \given \decision \rpar,
    \end{align}
    where $\kappa < \infty$ is the normalizing factor. Since both $\mu^\star_\decision(\cdot)$ and $M_{\cdot}\lpar r, o \given \decision \rpar$ belong to $W^{1,\alpha}\lpar \Theta_\decision \rpar$ for $\alpha \geq 2$, we can use Theorem 6.1 in \cite{behzadan2021multiplication} to conclude that $\mu^\star_\decision(\cdot) M_{\cdot}\lpar r, o \given \decision \rpar \in W^{1,\alpha}\lpar \Theta_\decision \rpar$. Applying this step for multiple times proves that $\mu_{\decision,t}^\star(\cdot) \in W^{1,\alpha}\lpar \Theta_\decision \rpar$. The proof for $\mu^\unif_{\decision,t}$ follows similar steps since $\mu^\unif_\decision \in W^{1,\infty}(\Theta_\decision) \subset  W^{1,\alpha}(\Theta_\decision)$. Given that  $\mu^\unif_{\decision,t}, \mu_{\decision,t}^\star \in W^{1,\alpha}(\Theta_\decision)$, we can directly apply Theorem 2.1 in \cite{chae2020wasserstein} to conclude \cref{eq:wass-tv}.
\end{proof}
Our reason to choose the Wasserstein distance is the recent line of work that provides bounds on the Wasserstein distance between posterior distributions under different priors~\citep{ley2017distances,mijoule2023stein}. In particular, we can use Corollary 3.4 in \cite{ley2017distances} to get the following:
\begin{align}
    \wass{\mu^\unif_{\decision,t}}{\mu_{\decision,t}^\star} \leq \left\|(\mu^\star_\decision)'\right\|_\infty \var^\unif_{t}\lpar \theta_\decision \rpar, \label{eq:wass-post}
\end{align}
where $\var^\unif_{t}$ is the variance of $\theta_\decision$ after observing $h_{t-1}$ under prior $\mu^\unif$. Combining \cref{eq:tv-product,eq:wass-tv,eq:wass-post}, we get
\begin{align}
    \tv{\mu^\unif_t}{\mu_t^\star} &\leq c \sum_{\decision \in \decSpace} \lpar \left\|\mu^\unif_{\decision,t}\right\|_{W^{1,\alpha}} + \left\|\mu^\star_{\decision,t}\right\|_{W^{1,\alpha}}\rpar^{\frac{1}{\alpha+1}} \lpar\left\|(\mu^\star_\decision)'\right\|_\infty \var^\unif_{t}\lpar \theta_\decision \rpar\rpar^{\frac{\alpha}{\alpha + 1}} \\
    & \leq c (B')^{\frac{1}{\alpha+1}} \sum_{\decision \in \decSpace} \lpar \left\|\mu^\unif_{\decision,t}\right\|_{W^{1,\alpha}} + \left\|\mu^\star_{\decision,t}\right\|_{W^{1,\alpha}}\rpar^{\frac{1}{\alpha+1}} \lpar\var^\unif_{t}\lpar \theta_\decision \rpar\rpar^{\frac{\alpha}{\alpha + 1}} \tag*{By \cref{assump:smooth-prior}}\\
    & \leq C(B')^{\frac{1}{\alpha+1}}\sum_{\decision \in \decSpace} \lpar\var^\unif_{t}\lpar \theta_\decision \rpar\rpar^{\frac{\alpha}{\alpha + 1}} \label{eq:tv-var}
\end{align}
\vahidcomment{In the last inequality, I assumed $\lpar \left\|\mu^\unif_{\decision,t}\right\|_{W^{1,\alpha}} + \left\|\mu^\star_{\decision,t}\right\|_{W^{1,\alpha}}\rpar^{\frac{1}{\alpha+1}}$ is bounded. It needs more caution.} Given \cref{eq:tv-var} and that $\var^\unif_{t}(\theta_\decision) = \cO\lpar {n_t(\decision)}^{-\beta} \rpar$, we have
\begin{align}
    \E \lbar \sum_{t=1}^T \tv{\mu^\unif_t}{\mu_t^\star}\rbar \lesssim \sum_{t=1}^T \sum_{\decision \in \decSpace} \lpar\frac{1}{n_t(\decision)}\rpar^{\frac{\beta \alpha}{\alpha + 1}} 
\end{align}
\end{proof}

==> sections/temp.tex <==
We start by simplifying \cref{eq:bayes-regret}:
{\small
\begin{align}
     \bregret &= \E \lbar \sum_{t=1}^T f^\theta(a_\theta) -  \E \lbar f^\theta(a^t)\rbar \rbar\\
     &= \E \lbar \sum_{t=1}^T \E_t \lbar f^\theta(a_\theta)-  \E \lbar f^\theta(a^t)\rbar \rbar \rbar \\
     &= \E \lbar \sum_{t=1}^T \E_t \lbar f^\theta(a_\theta)-  \sum_{a \in \cA} \pi^t(a) f^\theta(a) \rbar \rbar\\
     &= \E  \lbar \sum_{t=1}^T \sum_{a \in \cA} \mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \E_t\lbar f^\theta(a) \given a_\theta = a \rbar - \pi^t(a) \E_t \lbar f^\theta(a) \rbar \rbar
\end{align}
}%
Adding and subtracting $\mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \E_t\lbar f^\theta(a) \rbar$ to the sum above, we get
{\small
\begin{align}
     \bregret
     &= \underbrace{\E  \lbar \sum_{t=1}^T \sum_{a \in \cA}  \lpar \mu_\star\lpar a_\theta = a \given h_{t-1} \rpar - \pi^t(a) \rpar  \E_t\lbar f^\theta(a) \rbar \rbar}_{\text{I}} + \underbrace{\E  \lbar \sum_{t=1}^T \mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \lpar \E_t\lbar f^\theta(a) \given a_\theta = a \rbar - \E_t \lbar f^\theta(a) \rbar \rpar  \rbar}_{\text{II}}
\end{align}
}%
\xhdr{Bounding term I} 
{\small
\begin{align}
     &\leq \E  \lbar \sum_{t=1}^T \left|\sum_{a \in \cA}  \lpar \mu_\star\lpar a_\theta = a \given h_{t-1} \rpar - \pi^t(a) \rpar  \E_t\lbar f^\theta(a) \rbar \right| + \left|\sum_{a \in \cA} \mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \lpar \E_t\lbar f^\theta(a) \given a_\theta = a \rbar - \E_t \lbar f^\theta(a) \rbar \rpar \right|\rbar \\
     & \leq \sum_{t=1}^T \E \lbar \tv{\mu_\star\lpar \cdot \given h_{t-1} \rpar}{\pi^t}\rbar + \E  \lbar \sum_{t=1}^T \left|\sum_{a \in \cA} \mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \lpar \E_t\lbar f^\theta(a) \given a_\theta = a \rbar - \E_t \lbar f^\theta(a) \rbar \rpar\right| \rbar \tag{Since $f^\theta \in [0, 1]$} \\
      & = \sum_{t=1}^T \E \lbar \tv{\mu_\star\lpar \cdot \given h_{t-1} \rpar}{\pi^t}\rbar + \E  \lbar \sum_{t=1}^T \left|\sum_{a \in \cA} \sqrt{\frac{\mu_\star\lpar a_\theta = a \given h_{t-1} \rpar}{\pi^t(a)}} \sqrt{\mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \pi^t(a)} \lpar \E_t\lbar f^\theta(a) \given a_\theta = a \rbar - \E_t \lbar f^\theta(a) \rbar \rpar\right| \rbar \tag{Assuming $\mu_\star\lpar \cdot \given h_{t-1} \rpar \ll \pi^t$}\\
      & \stackrel{(a)}{\leq}  \sum_{t=1}^T \E \lbar \tv{\mu_\star\lpar \cdot \given h_{t-1} \rpar}{\pi^t}\rbar + \E  \lbar \sum_{t=1}^T \sqrt{\sum_{a \in \cA} {\frac{\mu_\star\lpar a_\theta = a \given h_{t-1} \rpar}{\pi^t(a)}}} \cdot \sqrt{\sum_{a \in \cA} {\mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \pi^t(a)} \lpar \E_t\lbar f^\theta(a) \given a_\theta = a \rbar - \E_t \lbar f^\theta(a) \rbar \rpar^2} \rbar \label{eq:help-bregret}
\end{align}
}%
Where (a) follows form the Cauchy-Schwarz inequality. We further simplify the R.H.S of the above inequality. Note that,
\begin{align}
    \E_t\lbar f^\theta(a) \given a_\theta = a \rbar - \E_t \lbar f^\theta(a) \rbar  &= \E_t\lbar r^t \given a_\theta = a, a^t = a \rbar - \E_t \lbar r^t \given a^t = a \rbar \\
    & \stackrel{(a)}{\leq} \sqrt{\frac12 \kl{\mu_t\lpar r^t \given a_\theta = a, a^t = a\rpar}{\mu_t\lpar r^t \given a^t = a\rpar}} \label{eq:pinsker-bregret}
\end{align}
where (a) follows from Pinsker's inequality. Combining \cref{eq:help-bregret,eq:pinsker-bregret} and defining $\Gamma_t := \sum_{a \in \cA} {\frac{\mu_\star\lpar a_\theta = a \given h_{t-1} \rpar}{\pi^t(a)}}$, we get
{\small
\begin{align}
    \bregret & \leq \sum_{t=1}^T \E \lbar \tv{\mu_\star\lpar \cdot \given h_{t-1} \rpar}{\pi^t}\rbar + \E  \lbar \sum_{t=1}^T \sqrt{\Gamma_t} \cdot \sqrt{\sum_{a \in \cA} {\mu_\star\lpar a_\theta = a \given h_{t-1} \rpar \pi^t(a)} \kl{\mu_t\lpar r^t \given a_\theta = a, a^t = a\rpar}{\mu_t\lpar r^t \given a^t = a\rpar} } \rbar \\
    & \stackrel{(a)}{\leq} \sum_{t=1}^T \E \lbar \tv{\mu_\star\lpar \cdot \given h_{t-1} \rpar}{\pi^t}\rbar + \E  \lbar \sum_{t=1}^T \sqrt{\Gamma_t} \cdot \sqrt{I_t\lpar a_\theta ; a^t, r^t\rpar} \rbar \\
    & \stackrel{(b)}{\leq} \sum_{t=1}^T \E \lbar \tv{\mu_\star\lpar \cdot \given h_{t-1} \rpar}{\pi^t}\rbar + \sqrt{\E  \lbar \sum_{t=1}^T {\Gamma_t}\rbar} \cdot \sqrt{ \E \lbar{\sum_{t=1}^T I_t\lpar a_\theta ; a^t, r^t\rpar} \rbar} \\
    & \stackrel{(c)}{\leq} \sum_{t=1}^T \E \lbar \tv{\mu_\star\lpar \cdot \given h_{t-1} \rpar}{\pi^t}\rbar + \sqrt{\E  \lbar \sum_{t=1}^T {\Gamma_t}\rbar} \cdot \sqrt{H(a_\theta)} 
\end{align}
}%
where $I_t\lpar a_\theta ; a^t, r^t\rpar$ is the mutual information between the optimal policy $a_\theta$ and the observed action/reward at time $t$ under the posterior distribution, $H(a_\theta)$ is the entropy of the optimal policy under the prior distribution, and (b) follows from the Cauchy-Schwarz inequality.\vahidcomment{Explain why (a), (c) holds in more detail - For now, I refer it to Proposition 1 and 2 from \citet{russo2016information}}

